Constructions for Quantum Indistinguishability Obfuscation

An indistinguishability obfuscator is a probabilistic polynomial-time algorithm that takes a circuit as input and outputs a new circuit that has the same functionality as the input circuit, such that for any two circuits of the same size that compute the same function, the outputs of the indistinguishability obfuscator are indistinguishable. Here, we study schemes for indistinguishability obfuscation for quantum circuits. We present two definitions for indistinguishability obfuscation: in our first definition (qiO) the outputs of the obfuscator are required to be indistinguishable if the input circuits are perfectly equivalent, while in our second definition (qiOD), the outputs are required to be indistinguishable as long as the input circuits are approximately equivalent with respect to a pseudo-distance D. Our main results provide (1) a computationally-secure scheme for qiO where the size of the output of the obfuscator is exponential in the number of non-Clifford (T gates), which means that the construction is efficient as long as the number of T gates is logarithmic in the circuit size and (2)a statistically-secure qiOD, for circuits that are close to the kth level of the Gottesman-Chuang hierarchy (with respect to D); this construction is efficient as long as k is small and fixed.

==> qPQfromiO.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Section
\section{Quantum Public-Key Encryption from iO}
\label{sec:Quantum-public-key}
Here, \emph{quantum public-key encryption} refers to the  encryption of a quantum register using a classical public key, see Section~\ref{sec:prelim-quantum-PKE} for related definitions.


\subsection{Obfuscation-based Scheme}
The scheme is based on an idea for ``classical public-key encryption based from indistinguishability obfuscation'' see~\cite{SW14}.
\label{sec:obfuscation}
\begin{itemize}
\item Common Parameters:
\begin{enumerate}
\item Let  ${\rm G}: \{0,1\}^n\rightarrow \{0,1\}^{2n}$ be a quantum secure pseudorandom number generator.
\item Let  $F_k:\{0,1\}^{2n} \times \{0,1\}^{2n} \longrightarrow \{0,1\}^{2n}$ be a quantum secure puncturable pseudorandom function.
\item Let $qi\mathcal{O}$ be a quantum secure classical indistinguishability obfuscation
\item Plaintext space  $\mathcal{D}(\mathcal{H}_{M}),$ where $M=2n$ and Ciphertext space $\mathcal{H}_C=\mathcal{D}(\mathcal{H}_{M})\otimes \mathcal{D}(\mathcal{H}_{M}).$
\end{enumerate}
\end{itemize}

\begin{itemize}
\item ${\rm KeyGen}(1^n)$
\begin{enumerate}
\item  Pick a random key $k\rightarrow \{0,1\}^{2n}$ and set $k$ as the puncturable qPRF key.
\item Construct  program $P_k(s)$ that takes an $n$ bit string as an input and the key $k$ is hardcoded in $P_k.$
\begin{itemize}
\item[] $P_k(s) \{$
\begin{itemize}
\item[] $r\leftarrow {\rm G}(s)$
\item[] $y \leftarrow F_k(r)$
\item[] return $(r,y).$
\end{itemize}
\item[] \}
\end{itemize}
\item Set public key $pk=qi\mathcal{O}(P_k,1^n)$ and the secret key $sk=k.$
\item Output $(pk,sk).$
\end{enumerate}
\end{itemize}


\begin{itemize}
\item ${\rm Enc}(qi\mathcal{O}(P_k,1^n), \rho):$
\begin{enumerate}
\item Pick a random string $s\rightarrow \{0,1\}^n.$
\item Set $(y,r)=qi\mathcal{O}(P_k,1^n)(s).$
\item  Output the ciphertext $\ket{r}\bra{r} \otimes P_y \rho P_y.$
\end{enumerate}
\end{itemize}

\begin{itemize}
\item ${\rm Dec}(k, \sigma):$
\begin{enumerate}
\item Measure the first $2n$ qubits in the computational basis to obtain $r^\prime \in \{0,1\}^n.$
\item Compute $y^\prime=F_k(r^\prime).$
\item Output the plaintext $P_{y^\prime}\sigma P_{y^\prime}.$
\end{enumerate}
\end{itemize}

\begin{theorem}
If $G$ is a quantum secure qPRNG, $F_k$ is a quantum secure puncturable qPRF  and $qi\mathcal{O}$ is quantum secure classical obfuscator, then Scheme \ref{sec:obfuscation} is an IND-CPA secure
 quantum public key encryption scheme.
\end{theorem}

\noindent{\bf Proof}. Our proof is consists of a sequence of hybrid experiments where the first hybrid corresponds to the
IND-CPA experiment, in which a challenger{\em C} interacts with a polynomial-time adversary $\mathcal{A}=(\mathcal{A}_1, \mathcal{A}_2).$ We prove that adversaries's advantage must be the negligibly close between each successive hybrid and that the adversary has zero advantage in the last experiment. Hence, concluding that for any polynomial-time adversary the advantage of winning IND-CPA  experiment is at most negligible.

\begin{itemize}
\item ${\bf Hybrid_0}$
\begin{enumerate}
\item {\em C} generates pair of secret/ public keys $(k, qi\mathcal{O}(P_k)) \leftarrow{\rm KeyGen}(1^n).$
\item $\mathcal{A}_1$ obtained the public-key $qi\mathcal{O}(P_k)$ from {\em C}
\item $\mathcal{A}_1$ outputs a quantum state  $\rho_{ME}$ on  $\mathcal{D}(\mathcal{H}_{2n}) \otimes \mathcal{E}.$
\item {\em C} computes $c_0={\rm Enc}(pk,\ket{0}\bra{0}_\mathcal{M}), c_1={\rm Enc}(pk,\rho_M),$ $r^* \xleftarrow[]{\$} \bit{}$ and outputs $c_i=\ket{r}\bra{r} \otimes P_y \rho P_y,$ where $\rho=\ket{0}\bra{0}_\mathcal{M}$ if $i=0$ and  $\rho=\rho_M$ otherwise.
\item  $\mathcal{A}_2$ obtains the challenge ciphertext $\ket{r}\bra{r} \otimes P_y \rho P_y$ from{\em C} and $\rho_E$ from $\mathcal{A}_1.$
\end{enumerate}
\end{itemize}

\begin{itemize}
\item${\bf Hybrid_1} \hspace{-0.12cm}:$ This hybrid is similar to $\mbox{Hybrid}_0$ except the ciphertext is given as $\ket{r^*}\bra{r^*} \otimes P_{f_k(r^*)} \rho P_{f_k(r^*)},$ where $r^* \xleftarrow[]{\$} \bit{2n}.$
\begin{enumerate}
\item {\em C} generates pair of secret/public keys $(k, qi\mathcal{O}(P_k)) \leftarrow{\rm KeyGen}(1^n).$
\item $\mathcal{A}_1$ obtained the public-key $qi\mathcal{O}(P_k)$ from{\em C}
\item $\mathcal{A}_1$ picks a quantum state  $\rho_{ME}$ on  $\mathcal{D}(\mathcal{H}_{2n}) \otimes \mathcal{E}$ and outputs $\rho_{M}.$
\item{\em C} picks $r^* \xleftarrow[]{\$} \bit{n},\, i \xleftarrow[]{\$} \bit{}$  and output the ciphertext $\ket{r^*}\bra{r^*} \otimes P_{f_k(r^*)} \rho P_{f_k(r^*)},$ where $\rho=\ket{0}\bra{0}_\mathcal{M}$ if $i=0$ and  $\rho=\rho_M$ otherwise.
\item  $\mathcal{A}_2$ obtains the challenge ciphertext $\ket{r^*}\bra{r^*} \otimes P_{f_k(r^*)} \rho P_{f_k(r^*)}$ from{\em C} and $\rho_E$ from $\mathcal{A}_1.$
\end{enumerate}
\end{itemize}



\begin{itemize}
\item ${\bf Hybrid_2}:$ In this hybrid we replace the public key in hybrid 1 by the obfuscation of the program $P_{k\{r^*\}}$ (define below).
\begin{enumerate}
\item{\em C} picks a random key $k\rightarrow \{0,1\}^{2n}$ and constructs a program $P_{k\{r^*\}}.$
\begin{itemize}
\item[] $P_{k\{r^*\}}(s) \{$
\begin{itemize}
\item[] $r\leftarrow {\rm G}(s)$
\item[] $y \leftarrow \textsf{Eval}_F(k\{r^*\},r)$
\item[] return $(r,\textsf{Eval}_F(k\{r^*\}).$
\end{itemize}
\item[] \}
\end{itemize}
 \item Set the secret key $sk=k$ and the public key $pk^*=qi\mathcal{O}(P_{k\{r^*\}},1^n).$
 \item  $\mathcal{A}_1$ obtains $pk$ from{\em C} and outputs a quantum state  $\rho_{ME}$ on $\mathcal{D}(\mathcal{H}_{2n}) \otimes \mathcal{E}.$
 \item {\em C} picks $s\xleftarrow[]{\$} \bit{2n}$ and obtain $(r,y)= qi\mathcal{O}(P_{k\{r^*\}},1^n)(s).$
 \item{\em C} picks $r^* \xleftarrow[]{\$} \bit{n},\, i \xleftarrow[]{\$} \bit{}$ and output the ciphertext $c_i=\ket{r^*}\bra{r^*} \otimes P_y \rho P_y,$ where $\rho=\ket{0}\bra{0}_\mathcal{M}$ if $i=0$ and  $\rho=\rho_M$ otherwise.
\item  $\mathcal{A}_2$ obtains the challenge ciphertext $\ket{r^*}\bra{r^*} \otimes P_y \rho P_y$ from{\em C} and $\rho_E$ from $\mathcal{A}_1.$
\end{enumerate}
\end{itemize}

\begin{itemize}
\item ${\bf Hybrid_3}\hspace{-0.09cm}:$ This hybrid is similar to $\mbox{Hybrid}_2$ except the ciphertext is given as $\ket{r^*}\bra{r^*} \otimes P_{y^*} \rho P_{y^*}.$ Where $y^* \xleftarrow[]{\$} \bit{2n}.$
\end{itemize}

\begin{itemize}
\item ${\bf Hybrid_0}$ and ${\bf Hybrid_1}\hspace{-0.09cm}:$ If there is a polynomial-time quantum adversary can distinguish between the two hybirds, then there exists a  polynomial-time quantum adversary that can break the security of PRNG. Suppose $\mathcal{A}$ on input  $\ket{G(s)}\bra{G(s)} \otimes P_{G(s)} \rho P_{G(s)}$  outputs 0 and on input $\ket{r^*}\bra{r^*} \otimes P_{f_k(r^*)} \rho P_{f_k(r^*)}$  outputs 1 with non-negligible advantage, then we construct polynomial-time quantum adversary $\mathcal{B}$ that can break the security of PRNG G.

 \begin{enumerate}
\item $\mathcal{B}$ runs the PRNG experiment and obtain a challenge $z.$
\item $\mathcal{B}$ then runs  $\mbox{Hybrid}_0$ and obtain the plaintext $\rho_M.$
\item $\mathcal{B}$ picks a random bit $i \xleftarrow[]{\$} \bit{}$ and sets the ciphertext $c_i=\ket{z}\bra{z} \otimes P_z \rho P_z,$ where $\rho=\ket{0}\bra{0}_\mathcal{M}$ if $i=0$ and  $\rho=\rho_M$ otherwise.
\item  $\mathcal{B}$ runs $\mathcal{A}$ on the input $c_i.$ If $\mathcal{A}$ outputs bit $j,$ then $\mathcal{B}$ outputs $j.$ Note $j=0$ corresponds to ${\bf Hybrid_o}$ which means $z$ is the output of PRNG and $j=1$ corresponds to ${\bf Hybrid_1}$ which means $z$ is randomly picked. Therefore, if $\mathcal{A}$ exist then we can construct $\mathcal{B}$ breaks the security of Puncturable PRF with non-negligible advantage.
\end{enumerate}
\end{itemize}




\begin{itemize}
\item ${\bf Hybrid_1}$ and ${\bf Hybrid_2}\hspace{-0.09cm}:$ In both of these hydrids $r^*$ is picked randomly. All we have to show that  $P_{k\{r^*\}}$ and $P_{k}$ have same functionality. Note if $r^*\notin \{G(s) \mid s\in \{0,1\}^n\}$ then both $P_{k\{r^*\}}$ and $P_{k}$ will have the same functionality. When $r^*$ is picked randomly from $\bit{2n}$ then with probability $\frac{1}{2^n},$  $r^*\in \{G(s) \mid s\in \{0,1\}^n\}$ is $1-\frac{1}{2^n}.$ Therefore with overwhelming probability both programs will have same functionality. We can apply apply iO security to conclude that $qi\mathcal{O}(P_k,1^n)$ and $qi\mathcal{O}(P_{k\{r^*\}},1^n)$ are computationally indistinguishable.
\end{itemize}


\begin{itemize}
\item ${\bf Hybrid_2}$ and ${\bf Hybrid_3}\hspace{-0.09cm}:$ The ciphertext in $\mbox{Hybrid}_2$ is given as $$\ket{r^*}\bra{r^*} \otimes P_{f_k(r^*)} \rho P_{f_k(r^*)}$$ and the ciphertext in $\mbox{Hybrid}_3$ is given as $$\ket{r^*}\bra{r^*} \otimes P_{y^*} \rho P_{y^*},$$ where $r^*\xleftarrow[]{\$} \bit{2n}$ and $y^*\xleftarrow[]{\$} \bit{2n}.$ If there exists is a polynomial-time adversary $\mathcal{A}$ that can distinguish between the two hybrids with non-negligible advantage, i.e

\[
    \mathcal{A}(1^n, (\ket{r^*}\bra{r^*} \otimes P_{y} \rho P_{y} ))=
\begin{cases}
    0, & \text{if } y\xleftarrow[]{\$} \bit{2n}.\\
    1, & \text{if }  y=F_k(r^*),
\end{cases}
\]
then we can construct a polynomial time adversary $\mathcal{B}$ that can break the Puncturable PRF security.

\begin{enumerate}
\item $\mathcal{B}$ picks a random secret key $k\rightarrow \{0,1\}^{2n}$ and set public key as  $qi\mathcal{O}(P_{k\{r^*\}},1^n).$
\item $\mathcal{B}$ runs the experiment $\textsf{PunctPRF}_{D,F}(n)$ and obtain $(k\{r^*\}, y),$ where $y=f_k(r^*)$ or $y=y\xleftarrow[]{\$} \bit{2n}.$
\item $\mathcal{B}$ then  run  $\mbox{Hybrid}_2$  and obtain the ciphertext $\ket{r^*}\bra{r^*} \otimes P_{f_k(r^*)} \rho P_{f_k(r^*)}.$
\item $\mathcal{B}$ creates modified ciphertext  as $\ket{r^*}\bra{r^*} \otimes P_{y} \rho^\prime P_{y}.$
\item  $\mathcal{B}$ runs $\mathcal{A}$ on the input  $\ket{r^*}\bra{r^*} \otimes P_{y} \rho^\prime P_y.$
\item $\mathcal{B}$ outputs whatever the bit outputs by $\mathcal{A}.$  Note if $y$ is the value of PRF at the punctured point, then we are in hybrid 2 and $\mathcal{A}$ outputs 1 with non-negligible advantage. Otherwise $y$ is random and we are in hybrid 3 and $\mathcal{A}$ outputs 0 with non-negligible advantage. Therefore, $\mathcal{B}$ breaks the security of Puncturable PRF.
\end{enumerate}
\end{itemize}

\begin{itemize}
\item ${\bf Hybrid_3}\hspace{-0.09cm}:$ The ciphertext in this experiment leaks no information about the plaintext. Since the advantage of all polynomial-time attacker's are negligibly close in each successive hybrid, this proves that the  scheme \ref{sec:obfuscation} is IND-CPA secure.
\end{itemize}

\subsection{Instantiation of Quantum Public-Key Cryptosystems}

{\color{red} So far all seems to be broken. Need to work on this.}
%This scheme is based on an idea for ``classical public-key encryption based from indistinguishability obfuscation'' (see Sahai and Water. \emph{How to Use Indistinguishability Obfuscation: Deniable Encryption, and More} \url{https://eprint.iacr.org/2013/454.pdf}).
%
%The public key consists in an obfuscation of $f(r) = (PRG(r), PRF(K, PRG(r))$, where $PRF$ is a pseudo-random function, $PRG$ is a pseudo-random generator.
%
%The encryption procedure consists in computing:  $a = PRF(K, PRG(x))$ and $b =   PRF(K, PRG(y))$ for randomly-chosen $x, y$.
%
%Next, we encrypt register $R$ with $Z^a Z^b$. The full ciphertext consists in $PRG(x), PRG(y)$ as well as register $R$.
%
%The security of this scheme depends on the existence of a quantum-secure \emph{indistinguishability obfuscator}, as well as on the $PRF$ and $PRG$, I guess.
%
%Actually, the scheme can be more abstractly defined as Section 5.1 of Sahai-Waters. The description above follows along the lines of the more intuitive description they give in the introduction.
%
%The proof, I anticipated would consists in a nice hybrid argument, using a technique of \emph{puncture programs} as introduced by Sahai-Waters. All of this would need to be adapted to the quantum case, see their Theorem 4.

